CycleNet: Rethinking Cycle Consistency in Text-Guided Diffusion for Image Manipulation

Diffusion models (DMs) have enabled breakthroughs in image synthesis tasks but lack an intuitive interface for consistent image-to-image (I2I) translation. Various methods have been explored to address this issue, including mask-based methods, attention-based methods, and image-conditioning. However, it remains a critical challenge to enable unpaired I2I translation with pre-trained DMs while maintaining satisfying consistency. This paper introduces Cyclenet, a novel but simple method that incorporates cycle consistency into DMs to regularize image manipulation. We validate Cyclenet on unpaired I2I tasks of different granularities. Besides the scene and object level translation, we additionally contribute a multi-domain I2I translation dataset to study the physical state changes of objects. Our empirical studies show that Cyclenet is superior in translation consistency and quality, and can generate high-quality images for out-of-domain distributions with a simple change of the textual prompt. Cyclenet is a practical framework, which is robust even with very limited training data (around 2k) and requires minimal computational resources (1 GPU) to train. Project homepage: https://cyclenetweb.github.io/

==> figs/ablation.tex <==
\begin{figure*}[!htp]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/source/ablation.pdf}
    \caption{Ablation study.}
    \label{fig::ablation}
    \vspace*{-0.25cm}
\end{figure*}

==> sections/02-background.tex <==
\section{Related Work}

\subsection{Conditional Image Manipulation with Diffusion Models}

Building upon Diffusion Probabilistic Models~\citep{sohl2015deep,ho2020denoising,song2021denoising,dhariwal2021diffusion}, pre-trained Diffusion Models (DMs)~\citep{rombach2022high,ramesh2022hierarchical,saharia2022photorealistic} have achieved state-of-the-art performance in image generation tasks. 
Text prompts are the most common protocol to enable conditional image manipulation with DMs, which can be done by fine-tuning a pre-trained DM~\citep{kawar2022imagic,kim2022diffusionclip}.
Mask-based methods have also been proposed with the help of user-prompted/automatically generated masks~\citep{nichol2022glide,couairon2023diffedit,avrahami2023spatext} or augmentation layers~\citep{bar2022text2live}.
To refrain from employing additional masks, recent work has explored attention-based alternatives~\citep{hertz2022prompt,mokady2022null, li2023stylediffusion,parmar2023zero}.
They first invert the source images to obtain the cross-attention maps and then perform image editing with attention control.
The promising performance of these methods is largely dependent on the quality of attention maps, which cannot be guaranteed in images with complicated scenes and object relationships, leading to undesirable edits when performing image-to-image translation.
Very recently, additional image-conditioning has been explored to perform paired image-to-image translation, using a side network~\citep{zhang2023adding} or an adapter~\citep{mou2023t2i}.
In this work, we follow this line of research and seek to enable unpaired image-to-image translation with pre-trained DMs while maintaining a satisfactory level of consistency. 


\subsection{Unpaired Image-to-Image Translation}

Image-to-image translation (I2I) is a fundamental task in computer vision, which is concerned with learning a mapping across images of different domains. 
% I2I has many downstream applications, e.g., style transfer~\citep{gatys2016neural} and colorization~\citep{zhang2016colorful}.
Traditional GAN-based methods~\citep{isola2017image} along this line require instance-level paired data, which are difficult to collect in many domains.
To address this limitation, the unpaired I2I setting~\citep{zhu2017unpaired,liu2017unsupervised} was introduced to transform an image from the source domain $\mathcal{X}$ into one that belongs to the target domain $\mathcal{Y}$, given only unpaired images from each domain.
Several GAN-based methods~\citep{zhu2017unpaired,yi2017dualgan,liu2017unsupervised,huang2018multimodal,liu2019few} were proposed to address this problem.
In recent years, DPMs have demonstrated their superior ability to synthesize high-quality images, with several applications in I2I translation~\citep{sasaki2021unit,choi2021ilvr}.
% UNIT-DDPM~\citep{sasaki2021unit} trains two DMs and two translation functions.
% ILVR~\citep{choi2021ilvr} relies on a DPM trained on the target domain while guiding it with a low-pass filter over the perturbed source image. 
With the availability of pre-trained DMs, SDEdit~\citep{meng2021sdedit} changes the starting point of generation by using a noisy source image that preserves the overall structure. 
EGSDE~\citep{zhao2022egsde} combines the merit of ILVR and SDEdit by introducing a pre-trained energy function on both domains to guide the denoising process. 
While these methods result in state-of-the-art performance on multiple benchmarks, it remains an open challenge to incorporate the pre-trained DMs for high-quality image generation, and at the same time, to ensure translation consistency.
% While there exist zero-shot methods~\citep{hertz2022prompt,mokady2022null,parmar2023zero}, they cannot leverage the source domain images for domain-specific applications. 


\subsection{Cycle Consistency in Image Translation}

The idea of cycle consistency is to regularize pairs of samples by ensuring transitivity between the forward and backward translation functions~\citep{sethi1987funding,pan2009recurrent, kalal2010forward}.
In unpaired I2I translation where explicit correspondence between source and target domain images is not guaranteed, cycle consistency plays a crucial role~\citep{zhu2017unpaired,kim2017learning,liu2017unsupervised,yi2017dualgan,torbunov2023uvcgan}.
Several efforts were made to ensure cycle consistency in diffusion-based I2I translation.
DDIB~\citep{su2022dual} proposed a theoretically solid approach for paired I2I translation with cycle consistency.
UNIT-DDPM~\citep{sasaki2021unit} made an initial attempt in the unpaired I2I setting, training two DPMs and two translation functions from scratch.
Cycle consistency losses are introduced in the translation functions during training to regularize the reverse processes.
At inference time, the image generation does not depend on the translation functions, but only on the two DPMs in an iterative manner, leading to sub-optimal performance.
Cycle Diffusion~\citep{wu2022unifying} proposes a zero-shot approach for image translation based on the observation that a certain level of consistency could emerge from DMs, and there is no explicit treatment to encourage cycle consistency.
To the best of our knowledge, \cyclenet~is the first diffusion-based method that guarantees cycle consistency in unpaired image-to-image translation with a simple trainable network and competitive performance.

